Counting Subgraphs in Somewhere Dense Graphs

We study the problems of counting copies and induced copies of a small pattern graph $H$ in a large host graph $G$. Recent work fully classified the complexity of those problems according to structural restrictions on the patterns $H$. In this work, we address the more challenging task of analysing the complexity for restricted patterns and restricted hosts. Specifically we ask which families of allowed patterns and hosts imply fixed-parameter tractability, i.e., the existence of an algorithm running in time $f(H)\cdot |G|^{O(1)}$ for some computable function $f$. Our main results present exhaustive and explicit complexity classifications for families that satisfy natural closure properties. Among others, we identify the problems of counting small matchings and independent sets in subgraph-closed graph classes $\mathcal{G}$ as our central objects of study and establish the following crisp dichotomies as consequences of the Exponential Time Hypothesis: (1) Counting $k$-matchings in a graph $G\in\mathcal{G}$ is fixed-parameter tractable if and only if $\mathcal{G}$ is nowhere dense. (2) Counting $k$-independent sets in a graph $G\in\mathcal{G}$ is fixed-parameter tractable if and only if $\mathcal{G}$ is nowhere dense. Moreover, we obtain almost tight conditional lower bounds if $\mathcal{G}$ is somewhere dense, i.e., not nowhere dense. These base cases of our classifications subsume a wide variety of previous results on the matching and independent set problem, such as counting $k$-matchings in bipartite graphs (Curticapean, Marx; FOCS 14), in $F$-colourable graphs (Roth, Wellnitz; SODA 20), and in degenerate graphs (Bressan, Roth; FOCS 21), as well as counting $k$-independent sets in bipartite graphs (Curticapean et al.; Algorithmica 19).

==> tikzlibraryconference.code.tex <==
%\documentclass{standalone}
%\usepackage{tikz}

\usepackage{ifthen}
\usetikzlibrary{calc,shapes,fit}
\usetikzlibrary{decorations.markings}


\tikzset{vertex/.style={circle, fill, inner sep=1pt, outer sep=1.3pt}}
\tikzset{svertex/.style={circle,draw=white, line width=1.2pt,fill=black, inner sep=1.8pt, outer sep=0pt}}
\tikzset{ssvertex/.style={circle,fill=black, inner sep=.7pt, outer sep=-.75pt}}
\tikzset{sssvertex/.style={circle,fill=black, inner sep=.5pt, outer sep=-.6pt}}
\tikzset{bbvertex/.style={circle,fill=black, inner sep=.8pt, outer sep=-.9pt}}
\tikzset{bag/.style={gray,minimum size=20pt,diamond,draw,rounded corners=4pt, inner sep=0pt, outer sep=-4pt, double=white, thick, fill=white}}
\tikzset{sbag/.style={gray,minimum size=15pt,diamond,draw,rounded corners=2pt, inner sep=0pt, outer sep=-4pt, double=white, thick, fill=white}}

%\tikzset{hom/.style={black}}
%\tikzset{shom/.style={white,double=black, thick}}

\def\ccol{red}
\def\ecol{blue}
\def\icol{red!50!blue}

\tikzset{ssedge/.style={white,thick, double=black, double distance=2pt}}
\tikzset{tedge/.style={white,thick, double=black, double distance=1pt}}
\tikzset{sssedge/.style={white,thick, double=black, double distance=1.5pt}}
\tikzset{stedge/.style={white,thin, double=gray, double distance=.6pt}}
\tikzset{sstedge/.style={white,thin, double=gray!60, double distance=.6pt}}
\tikzset{dedge/.style={gray,thick, double=white, double distance=9pt}}
\tikzset{sdedge/.style={gray,thick, double=white, double distance=5pt}}

\tikzset{sty/.store in=\sty,sty=10}

\tikzset{cross/.style={cross out, draw, minimum size=2*(#1-\pgflinewidth), inner sep=0pt, outer         sep=0pt}}

\tikzset{tvertex/.style={circle, fill, inner sep=1pt, outer sep=1.3pt}}
\tikzset{btvertex/.style={draw,circle,dashed,very thin,gray,inner sep=4pt, outer sep=-1pt}}
\tikzset{bbtvertex/.style={draw,dashed,thin,gray,inner sep=5.5pt, outer sep=-.5pt}}

\def\dotedge[#1](#2)--(#3);{%
    \draw[#1,dotted] ($(#2)!.33!(#3)$) -- ($(#2)!.66!(#3)$);%
    \draw[#1] ($(#2)!.64!(#3)$) -- (#3);%
    \draw[#1] (#2) -- ($(#2)!.35!(#3)$);%
}

%% slice from pgfpie

% #8:#1 center
% #7:#2 radius
% #1:#3 begin angle
% #2:#4 end angle
% #5:#5 explode
% #6: fill color

% #3: number
% #4: label
% #6: fill color

\makeatletter
\tikzset{slsty/.store in=\@sty,slsty=}
\def\slice#1#2#3#4#5#6#7{
    \pgfmathsetmacro{\midangle}{0.5*(#3)+0.5*(#4)}
    \pgfmathsetmacro{\sliceradius}{#2+#5}
    \path (#1) -- ++(\midangle:#5) coordinate(O);
    \node[inner sep=1pt, outer sep=1.2pt] (#7) at (O) {};
    \draw[line join=round, color=#6, fill=#6, \@sty] (O) -- ++(#3:#2) arc (#3:#4:#2) -- cycle;
}

% #1 coordinate
% #2 split
% #3 coordinate name
\def\kowaen#1#2#3;{
    \foreach \i/\j/\k [count=\c from 1] in {#2} {
        \slice{#1}{1.3pt}{\i}{\j}{2pt}{\k}{#3-\c};
    }
}

\def\coledge(#1|#2)--(#3|#4);{
    \draw[tedge] (#1) -- (#3);
    \draw[tedge, double=#2] (#1) -- ($(#1)!.35!(#3)$);
    \draw[tedge, double=#4] (#3) -- ($(#3)!.35!(#1)$);
}

\tikzset{
    every label/.append style={font=\tiny, label distance=-3}
}

\tikzset{
    pics/torus/.style args={#1/#2}{
        code = {
            \pgfmathsetmacro{\bg}{int(div(\sty,10))}
            \pgfmathsetmacro{\mode}{int(\sty - \bg * 10)}

            \pgfmathsetmacro{\normalgrid}{#2==14}
            \ifthenelse{\mode=0}{
                % normal mode
                \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                \ifthenelse{\normalgrid=1}{
                    \def\vs{tvertex}
                    }{
                    \def\vs{btvertex}
                }
                \def\es{tedge}
                \def\ess{stedge}
                }{
                \ifthenelse{\mode=1}{
                    % grid where each vertex is split into 6 parts (for a 3d grid
                    \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                    \ifthenelse{\normalgrid=1}{
                        \def\vs{tvertex}
                        }{
                        \def\vs{bbtvertex}
                    }
                    \def\es{tedge}
                    \def\ess{stedge}
                    }{
                    % grid-colored graph (only supports 2d grids
                    \pgfmathsetmacro{\dist}{\bg==2?1.15:.9}
                    \def\vs{bag}
                    \def\es{dedge}
                    \def\ess{sdedge}
                }
            }
            \pgfmathsetmacro{\n}{int(#1-1)}

            \foreach\j in {1,...,#1} {
                \pgfmathsetmacro{\xodd}{isodd(\j) && \j > 1 && \j <= \n}
                \pgfmathsetmacro{\xeven}{iseven(\j) && \j > 1 && \j <= \n}
                \ifthenelse{\xodd=1}{
                    \node[rotate=8,regular polygon,regular polygon sides=#1,minimum
                    size=\j*35pt] (p\j) {};
                    }{
                    \ifthenelse{\xeven=1}{
                        \draw[\es,double=black!20] circle (\j*17.6pt);
                        \node[rotate=-10/\j,regular polygon,regular polygon sides=#1,minimum
                        size=\j*35pt] (p\j) {};
                        }{
                        \node[regular polygon,regular polygon sides=#1,minimum
                        size=\j*35pt] (p\j) {};
                    }
                }

                \foreach\l in {1,...,#1}{
                    \pgfmathsetmacro{\de}{(9 * \l + 7.4) * 40 / #1}
                    \pgfmathsetmacro{\dee}{(9 * \l + 6) * 40 / #1}
                    \draw[very thick,white] (\de:\j * 17.6pt) arc (\de:\dee:\j *17.6pt);
                    \draw[thick,dotted,black!20] (\de:\j * 17.6pt) arc (\de:\dee:\j *17.6pt);
                    \node[inner sep=1.8pt, circle,fill= white] (\j\l) at (p\j.corner \l) {};
                    \ifthenelse{\xeven=1}{
                        \node[\vs,black!20] (\j\l) at (p\j.corner \l) {};
                    }{}
                }
            }
            \foreach\j in {1,...,#1} {
                \foreach\l in {1,...,#1}{

                \pgfmathsetmacro{\xeven}{iseven(\j) && \j > 2}
                \pgfmathsetmacro{\xodd}{isodd(\j) && \j > 2}
                \pgfmathsetmacro{\jmt}{int(\j - 2)}
                \ifthenelse{\xeven=1}{
                    \dotedge[\es,double=black!20](\j\l)--(\jmt\l);
                }{}
                \ifthenelse{\xodd=1}{
                    \dotedge[\es,double=black](\j\l)--(\jmt\l);
                }{}
            }
            \dotedge[\es,double=black!20](#1\j)--(\n\j);
            \dotedge[\es,double=black!20](1\j)--(2\j);
        }
        \foreach\j in {1,...,#1} {
                \pgfmathsetmacro{\xeven}{iseven(\j) && \j > 1 && \j <= \n}
                \ifthenelse{\xeven=1}{}{
                    \draw[\es] circle (\j*17.6pt);
                    \foreach\l in {1,...,#1}{
                        \node[inner sep=1.8pt, circle,fill= white] (\j\l) at (p\j.corner \l) {};
                        \node[\vs] (\j\l) at (p\j.corner \l) {};
                        \ifthenelse{\j=1}{
                            \pgfmathsetmacro{\de}{(9 * \l + 9) * 40 / #1}
                            \pgfmathsetmacro{\dee}{(9 * \l + 4.5) * 40 / #1}
                            }{
                            \pgfmathsetmacro{\de}{(9 * \l + 7.5) * 40 / #1}
                            \pgfmathsetmacro{\dee}{(9 * \l + 6.1) * 40 / #1}
                        }
                        \draw[very thick,white] (\de:\j * 17.6pt) arc (\de:\dee:\j *17.6pt);
                        \draw[thick,dotted] (\de:\j * 17.6pt) arc (\de:\dee:\j *17.6pt);
                    }
                }
            }
        }
    }
}
\tikzset{
    pics/grid/.style args={#1/#2}{
        code = {
            \pgfmathsetmacro{\bg}{int(div(\sty,10))}
            \pgfmathsetmacro{\mode}{int(\sty - \bg * 10)}

            \pgfmathsetmacro{\normalgrid}{#2==14}
            \ifthenelse{\mode=0}{
                % normal mode
                \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                \ifthenelse{\normalgrid=1}{
                    \def\vs{tvertex}
                    }{
                    \def\vs{btvertex}
                }
                \def\es{tedge}
                \def\ess{stedge}
                }{
                \ifthenelse{\mode=1}{
                    % grid where each vertex is split into 6 parts (for a 3d grid
                    \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                    \ifthenelse{\normalgrid=1}{
                        \def\vs{tvertex}
                        }{
                        \def\vs{bbtvertex}
                    }
                    \def\es{tedge}
                    \def\ess{stedge}
                    }{
                    % grid-colored graph (only supports 2d grids
                    \pgfmathsetmacro{\dist}{\bg==2?1.15:.9}
                    \def\vs{bag}
                    \def\es{dedge}
                    \def\ess{sdedge}
                }
            }
            \pgfmathsetmacro{\n}{int(#1-1)}
            \foreach\i[count=\j from 1] in {-\n,...,\n}
            \foreach\k[count=\l from 1] in {-\n,...,\n}{
                \pgfmathsetmacro{\xedgee}{\i==\n}
                \pgfmathsetmacro{\yedgee}{\k==\n}
                \pgfmathsetmacro{\bodd}{isodd(\j) && isodd(\l)}
                \pgfmathsetmacro{\yodd}{isodd(\l)}
                \pgfmathsetmacro{\xodd}{isodd(\j)}
                \ifthenelse{\bodd=1}{
                    \node[\vs] (\j\l) at (\dist*\i,\dist*\k) {};
                    \ifthenelse{\xedgee=1}{
                        \draw[smooth,\ess]
                        (\j\l.east)
                        to ($(\j\l.east) + (.35, 0)$)
                        to[out=0, in=0] ($(\j\l.east) + (.35, -0.25)$)
                        to ($(1\l.west) - (.15, 0.25)$)
                        to[out=180,in=180] ($(1\l.west) - (.15, 0)$)
                        to (1\l.west)
                        ;
                    }{}
                    }{
                    \node[inner sep=1.3ex] (\j\l) at (\dist*\i,\dist*\k) {};
                    \ifthenelse{\yodd=1}{
                        \draw[dotted,\es] (\j\l.west) -- (\j\l.east);
                        }{
                        \ifthenelse{\xodd=1}{
                            \draw[dotted,\es] (\j\l.north) -- (\j\l.south);
                            }{
                }}}
            }
            \foreach\i[count=\j from 1] in {-\n,...,\n}
            \foreach\k[count=\l from 1] in {-\n,...,\n}{
                \pgfmathsetmacro{\yedgee}{\k==\n}
                \pgfmathsetmacro{\bodd}{isodd(\j) && isodd(\l)}
                \pgfmathsetmacro{\yodd}{isodd(\l)}
                \pgfmathsetmacro{\xodd}{isodd(\j)}
                \ifthenelse{\bodd=1}{
                    \node[\vs] (\j\l) at (\dist*\i,\dist*\k) {};
                    \ifthenelse{\yedgee=1}{
                        \draw[smooth,\ess]
                        (\j\l.north)
                        to ($(\j\l.north) + (0,.15)$)
                        to[out=90, in=90] ($(\j\l.north) + (.25, 0.15)$)
                        to ($(\j1.south) - (-.25, 0.35)$)
                        to[out=270,in=270] ($(\j1.south) - (0,.35)$)
                        to (\j1.south)
                        ;
                    }{}
                    }{
                    \node[inner sep=1.3ex] (\j\l) at (\dist*\i,\dist*\k) {};
                    \ifthenelse{\yodd=1}{
                        \draw[dotted,\es] (\j\l.west) -- (\j\l.east);
                        }{
                        \ifthenelse{\xodd=1}{
                            \draw[dotted,\es] (\j\l.north) -- (\j\l.south);
                            }{
                }}}
            }
            \foreach\i[count=\j from 1] in {-\n,...,\n}
            \foreach\k[count=\l from 1] in {-\n,...,\n}{
                \pgfmathsetmacro{\xedge}{\i==-\n || \i==\n}
                \pgfmathsetmacro{\yedge}{\k==-\n || \k==\n}
                \pgfmathsetmacro{\xedgee}{\i==\n}
                \pgfmathsetmacro{\yedgee}{\k==\n}
                \pgfmathsetmacro{\corner}{\xedge && \yedge}
                \pgfmathsetmacro{\edge}{\xedge || \yedge}

                \ifthenelse{\corner=1}{\def\tp{corner}}
                {\ifthenelse{\edge=1}{\def\tp{edge}}
                {\def\tp{inner}}}

                \pgfmathsetmacro{\bodd}{isodd(\j) && isodd(\l)}
                \pgfmathsetmacro{\yodd}{isodd(\l)}
                \pgfmathsetmacro{\xodd}{isodd(\j)}
                \ifthenelse{\bodd=1}{
                    \ifthenelse{\normalgrid=1}{
                        \node[\vs] (\j\l) at (\dist*\i,\dist*\k) {};
                        }{
                        \ifthenelse{\mode=0}{
                            \node[ssvertex] (n\j\l) at ($(\j\l.north)+(0,-.065)$) {};
                            \node[ssvertex] (e\j\l) at ($(\j\l.east)+(-.065,0)$) {};
                            \node[ssvertex] (s\j\l) at ($(\j\l.south)+(0,.065)$) {};
                            \node[ssvertex] (w\j\l) at ($(\j\l.west)+(.065,0)$) {};

                            % \draw[ssedge] (n\j\l) -- (s\j\l);
                            % \draw[ssedge] (s\j\l) -- (e\j\l);
                            }{
                            \node[sssvertex] (ne\j\l) at ($(\j\l.north east)+(-0.05,-.05)$) {};
                            \node[ssvertex] (n\j\l) at ($(\j\l.north)+(0,-.06)$) {};
                            \node[ssvertex] (e\j\l) at ($(\j\l.east)+(-.06,0)$) {};
                            \node[ssvertex] (s\j\l) at ($(\j\l.south)+(0,.06)$) {};
                            \node[ssvertex] (w\j\l) at ($(\j\l.west)+(.06,0)$) {};
                            \node[bbvertex] (sw\j\l) at ($(\j\l.south west)-(-0.05,-.05)$) {};

                            \ifthenelse{#2=15}{
                                \draw[tedge] (ne\j\l) -- (sw\j\l);
                                \draw[sssedge] (w\j\l) -- (n\j\l) -- (e\j\l) -- (s\j\l);
                            }{}
                            \ifthenelse{#2=16}{
                                \draw[tedge] (w\j\l) -- (ne\j\l);
                                \draw[sssedge] (n\j\l) -- (s\j\l);
                                \draw[tedge] (ne\j\l) -- (e\j\l) -- (sw\j\l) -- (w\j\l);
                                \node[ssvertex] (n\j\l) at ($(\j\l.north)+(0,-.06)$) {};
                            }{}
                            \ifthenelse{#2=17}{
                                \draw[tedge] (s\j\l) -- (ne\j\l);
                                \draw[sssedge] (w\j\l) -- (e\j\l);
                                \draw[tedge] (sw\j\l) -- (n\j\l) -- (ne\j\l)  (s\j\l) -- (sw\j\l);
                                \node[ssvertex] (e\j\l) at ($(\j\l.east)+(-.06,0)$) {};
                            }{}
                        }
                        \ifthenelse{#2=1}{\draw[ssedge] (n\j\l) -- (s\j\l);}{}
                        \ifthenelse{#2=2}{\draw[ssedge] (w\j\l) -- (e\j\l);}{}
                        \ifthenelse{#2=3}{\draw[ssedge] (n\j\l) -- (e\j\l);}{}
                        \ifthenelse{#2=4}{\draw[ssedge] (s\j\l) -- (e\j\l);}{}
                        \ifthenelse{#2=5}{\draw[ssedge] (n\j\l) -- (w\j\l);}{}
                        \ifthenelse{#2=6}{\draw[ssedge] (s\j\l) -- (w\j\l);}{}
                        \ifthenelse{#2=7}{\draw[ssedge] (n\j\l) -- (e\j\l);
                        \draw[ssedge] (s\j\l) -- (w\j\l);}{}
                        \ifthenelse{#2=8}{\draw[ssedge] (s\j\l) -- (e\j\l);
                        \draw[ssedge] (n\j\l) -- (w\j\l);}{}
                        \ifthenelse{#2=9}{
                            \draw[ssedge] (e\j\l) -- (w\j\l);
                            \draw[ssedge] (s\j\l) -- (n\j\l);
                        }{}
                        \ifthenelse{#2=10}{\draw[ssedge] (n\j\l) -- (e\j\l) -- (s\j\l);}{}
                        \ifthenelse{#2=11}{\draw[ssedge] (e\j\l) -- (s\j\l) -- (w\j\l);}{}
                        \ifthenelse{#2=12}{\draw[ssedge] (s\j\l) -- (w\j\l) -- (n\j\l);}{}
                        \ifthenelse{#2=13}{\draw[ssedge] (w\j\l) -- (n\j\l) -- (e\j\l);}{}

                    }
                    \ifthenelse{\j>1}{
                        \pgfmathsetmacro{\up}{int(\j-1)}
                        \pgfmathsetmacro{\upp}{int(\j-2)}
                        \draw[\es] (\up\l) -- (\j\l);
                        \draw[\es] (\upp\l) -- (\up\l);
                    }{}
                    \ifthenelse{\l>1}{
                        \pgfmathsetmacro{\left}{int(\l-1)}
                        \pgfmathsetmacro{\leftt}{int(\l-2)}
                        \draw[\es] (\j\left) -- (\j\l);
                        \draw[\es] (\j\left) -- (\j\leftt);
                    }{}

                }{}
            }
        }
    }
}

\tikzset{
    pics/gridgrid/.style args={#1/#2}{
        code = {
            \pgfmathsetmacro{\bg}{int(div(\sty,10))}
            \pgfmathsetmacro{\mode}{int(\sty - \bg * 10)}
            \begin{scope}[opacity=0.4]
                \begin{scope}[opacity=0.2]
                    \pic[sty=\bg1] (2) at (2, 2) {grid=#1/#2};
                \end{scope}
                \pic[sty=\bg1] (1) at (1, 1) {grid=#1/#2};
            \end{scope}
            \pic[sty=\bg1] (0) at (0, 0) {grid=#1/#2};

            \pgfmathsetmacro{\normalgrid}{#2==14}
            \pgfmathsetmacro{\n}{int(#1-1)}
            \ifthenelse{\mode=0}{
                % normal mode
                \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                \ifthenelse{\normalgrid=1}{
                    \def\vs{tvertex}
                    }{
                    \def\vs{btvertex}
                }
                \def\es{tedge}
                \def\ess{stedge}
                }{
                \ifthenelse{\mode=1}{
                    % grid where each vertex is split into 6 parts (for a 3d grid
                    \pgfmathsetmacro{\dist}{\bg==2?1.4:.6}
                    \ifthenelse{\normalgrid=1}{
                        \def\vs{tvertex}
                        }{
                        \def\vs{bbtvertex}
                    }
                    \def\es{tedge}
                    \def\ess{stedge}
                    }{
                    % grid-colored graph (only supports 2d grids
                    \pgfmathsetmacro{\dist}{\bg==2?1.15:.9}
                    \def\vs{bag}
                    \def\es{dedge}
                    \def\ess{sdedge}
                }
            }

            \definecolor{l2b}{rgb}{.6,.6,.6}
            \definecolor{l1b}{rgb}{.8,.8,.8}
            \foreach\i[count=\j from 1] in {-\n,...,\n}
            \foreach\k[count=\l from 1] in {-\n,...,\n}{
                \pgfmathsetmacro{\xedge}{\i==-\n || \i==\n}
                \pgfmathsetmacro{\yedge}{\k==-\n || \k==\n}
                \pgfmathsetmacro{\xedgee}{\i==\n}
                \pgfmathsetmacro{\yedgee}{\k==\n}
                \pgfmathsetmacro{\corner}{\xedge && \yedge}
                \pgfmathsetmacro{\edge}{\xedge || \yedge}

                \ifthenelse{\corner=1}{\def\tp{corner}}
                {\ifthenelse{\edge=1}{\def\tp{edge}}
                {\def\tp{inner}}}

                \pgfmathsetmacro{\bodd}{isodd(\j) && isodd(\l)}
                \pgfmathsetmacro{\yodd}{isodd(\l)}
                \pgfmathsetmacro{\xodd}{isodd(\j)}
                \ifthenelse{\bodd=1}{
                    \ifthenelse{\normalgrid=1}
                    {

                        \draw[\es,double=black!60,dotted]  ($(0\j\l)!0.35!(1\j\l)$) --
                        ($(0\j\l)!0.64!(1\j\l)$);
                        \draw[\es,double=black!30,dotted]  ($(1\j\l)!0.35!(2\j\l)$) --
                        ($(1\j\l)!0.64!(2\j\l)$);
                        \draw[\es,double=black] (0\j\l) -- ($(0\j\l)!0.37!(1\j\l)$);
                        \draw[\es,double=black!40] (1\j\l) -- ($(0\j\l)!0.62!(1\j\l)$);

                        \draw[\es,double=black!40] (1\j\l) -- ($(1\j\l)!0.37!(2\j\l)$);
                        \draw[\es,double=black!20] (2\j\l) -- ($(1\j\l)!0.62!(2\j\l)$);
                        \draw[smooth,\ess]
                        (2\j\l.north east)
                        to ($(2\j\l.north east) + (.15,.15)$)
                        to[out=45, in=45] ($(2\j\l.north east) + (.45, 0.15)$)
                        to ($(0\j\l.south west) - (-0.05, 0.25)$)
                        to[out=270-45,in=270-45] ($(0\j\l.south west) - (.25,.25)$)
                        to (0\j\l.south west)
                        ;
                        }{
                        \draw[\es,double=black!60,dotted]  ($(0\j\l)!0.35!(1\j\l)$) --
                        ($(0\j\l)!0.64!(1\j\l)$);
                        \draw[\es,double=black!30,dotted]  ($(1\j\l)!0.35!(2\j\l)$) --
                        ($(1\j\l)!0.64!(2\j\l)$);
                        \draw[\es,double=black] (0\j\l) -- ($(0\j\l)!0.37!(1\j\l)$);
                        \draw[\es,double=black!40] (1\j\l) -- ($(0\j\l)!0.62!(1\j\l)$);

                        \draw[\es,double=black!40] (1\j\l) -- ($(1\j\l)!0.37!(2\j\l)$);
                        \draw[\es,double=black!20] (2\j\l) -- ($(1\j\l)!0.62!(2\j\l)$);
                        \draw[smooth,sstedge]
                        ($(2\j\l.north east) - (.02,.02)$)
                        to ($(2\j\l.north east) + (.05,.05)$)
                        to[out=45, in=45] ($(2\j\l.north east) + (.35, 0.05)$)
                        to ($(0\j\l.south west) - (-0.15, 0.15)$)
                        to[out=270-45,in=270-45] ($(0\j\l.south west) - (.15,.15)$)
                        to (0\j\l.south west)
                        ;

                    }
                }{}
            }

        }
    }
}


\makeatother

